An Analysis of Attention via the Lens of Exchangeability and Latent Variable Models

With the attention mechanism, transformers achieve significant empirical successes. Despite the intuitive understanding that transformers perform relational inference over long sequences to produce desirable representations, we lack a rigorous theory on how the attention mechanism achieves it. In particular, several intriguing questions remain open: (a) What makes a desirable representation? (b) How does the attention mechanism infer the desirable representation within the forward pass? (c) How does a pretraining procedure learn to infer the desirable representation through the backward pass? We observe that, as is the case in BERT and ViT, input tokens are often exchangeable since they already include positional encodings. The notion of exchangeability induces a latent variable model that is invariant to input sizes, which enables our theoretical analysis. - To answer (a) on representation, we establish the existence of a sufficient and minimal representation of input tokens. In particular, such a representation instantiates the posterior distribution of the latent variable given input tokens, which plays a central role in predicting output labels and solving downstream tasks. - To answer (b) on inference, we prove that attention with the desired parameter infers the latent posterior up to an approximation error, which is decreasing in input sizes. In detail, we quantify how attention approximates the conditional mean of the value given the key, which characterizes how it performs relational inference over long sequences. - To answer (c) on learning, we prove that both supervised and self-supervised objectives allow empirical risk minimization to learn the desired parameter up to a generalization error, which is independent of input sizes. Particularly, in the self-supervised setting, we identify a condition number that is pivotal to solving downstream tasks.

==> approximation.tex <==
%!TEX root = iclr2023_conference.tex

\def\orth{\mathrm{orth}}
\def\Norm{\mathtt{norm}}
\def\ence{\mathtt{enc}}

%\section{Model}
%
%\subsection{Transformer}
%
%Problem formulation:
%
%dataset: $ \cD = \{(X_n, Y_n)\}_{i = 1}^{N} $, where $X_n \in \RR^{L_n \times d}$ is the input sequence and $Y_n \in \RR^{L_n \times d}$ is the output sequence. Note that we denote by $X = (x^1, x^2, \ldots, x^L)^\top$ and $Y = (y^1, y^2, \ldots, y^L)^\top$ the input and output sequences.
%
%
%Attention: query: $Q_n = X_n W^\tq$, key $ K_n = X_n W^\tk$, value: $V_n = X_n W^\tv$. Our model:
%\begin{align} \label{eq:attn-inv}
%	\att(Q, K, V) &=  A D^{-1} V,
%\end{align}
%where 
%\begin{align}
%	A = \fk (Q, K), \quad D = \fk (K, K) + \lambda I.
%\end{align}
%
%
%{\red Concentration assumption:}
%\begin{align}
%	\hat \EE[\phi(k)\phi(k)^T] = \frac{1}{L}\phi(K)^\top \phi(K) \rightarrow \cC^\phi_{K} \in \RR^{\infty \times \infty},
%\end{align}
%which can be viewed as an unbiased estimator of
%\begin{align}
%	\cC^\phi = \EE_K [\cC^\phi_{K}].
%\end{align}
%In what follows, we write $\Lambda = \cC^\phi + \lambda \cI$.
%We consider the feature vector such that
%\begin{align}
%	\fk(q, k) = \phi(q)^\top \Lambda^{-1} \phi(k) = \varphi(q)^\top \varphi(k)
%\end{align}
%and 
%\begin{align}
%	\tilde \fk(q, k) = \phi(q)^\top \phi(k).
%\end{align}
%Then, the conditional mean embedding with respect to $\tilde \fk$ in \eqref{eq:att12} can be approximated via
%\begin{align}
%	\text{CME-attn}(Q, K, V) &= \frac{1}{L}\phi(Q)  \biggl( \frac{1}{L}\phi(K)^\top \phi(K)  + \lambda \cI \biggr)^{-1} \phi(K)^\top \psi(V) \noend
%	&{\red\approx} \frac{1}{L}\phi(Q)  ( \cC_K^\phi + \lambda \cI )^{-1} \phi(K)^\top \psi(V) \noend
%	&{\red \approx} \frac{1}{L}\phi(Q)  ( \cC^\phi + \lambda \cI )^{-1} \phi(K)^\top \psi(V) \noend
%	&= \fk(Q, K) \psi(V) = \att(Q, K, V).
%\end{align}
%
%Question: given $\fk$, how to recover $\tilde \fk$?
%Let $\fk(q, k) = \varphi(q)^\top \varphi(k)$ and $\red \phi = \Lambda^{1/2} \varphi$. We see that 
%
%
%




\section{Approximation: Attention as Conditional Mean Embedding}
\label{sec:approx}
In what follows, we first show how the transformer exploits equivariance. Then, we study the attention, which is a key component in the transformer, and show it approximates the conditional mean embedding.

\subsection{How Does Transformer Exploit Equivariance?} \label{sec:invariant}

In practice, a variety of machine learning tasks aim to learn a sequence-to-sequence (seq2seq) mapping that outputs a representation sequence $Y \in \cY^L$ of the input sequence $X^L$. Here $L\in \NN_+$ is the sequence length. Without loss of generality, we assume that the input sequences have the same length. In a few tasks \citep{vaswani2017attention, dosovitskiy2020image}, an aggregation function generates an output from the representation sequence $Y$. In other tasks \citep{bibid}, the representation sequence if the output of interest. In \S\ref{sec:approx}, we focus on the latter case, while in \S\ref{sec:gen}, we extend to the former case.
For example, in natural language processing (NLP) the input sequence consists of word tokens, and in computer vision (CV) the input sequence consists of image patches. Since the input sequences includes the positional embeddings of each word token or image patch, we can view the input sequence as an unordered set, which motivates the design of a neural network that exploit the symmetry within the input sequence.
Throughout the paper, we use the terminology of ``sequence'' or ``set'' exchangeably.
Specifically, we characterize the class of mappings with such a symmetry via the following notion of equivariance.

%Transformer \citep{vaswani2017attention, dosovitskiy2020image} aims to parameterize a sequence to sequence (seq2seq) mapping from $ X \in \cX^L$ to $Y \in \cY^L$.
%
%We view transformer \citep{vaswani2017attention, dosovitskiy2020image} as a sequence to sequence mapping that maps a input sequence $ X \in \cX^L$ to an output sequence $Y \in \cY^L$.  We notice that with the presence of the positional embedding, this sequence to sequence mapping exploits the symmetry of the data. That is, when applying permutations to the sequence, the output of a transformer encoder does not change up to the same permutation. In what follows, we introduce the notion of equivariance for sequence to sequence mappings, which characterizes such symmetry.

\begin{definition}[Equivariance]
	\label{def:inv-eqv}
	We say that a seq2seq mapping $F: \cX^L \rightarrow \cY^L$ is equivariant if it holds that $ \pi(F(X)) = F(\pi(X)) $ for any permutation $\pi \in \SSS_L$, where $\SSS_{L}$ is the permutation group.
\end{definition}

Correspondingly, we define the following class of compositional equivariant mappings,
\begin{align}
	\label{eq:fc-tar}
	\cF^* = \{F = F_T \circ F_{T- 1} \circ \cdots \circ F_1 : \cX^L \rightarrow \cX^L \given \text{for any } t\in [T], F_t: \cX^L\rightarrow \cX^L \text{ is equivariant}\},
\end{align}
where $T \in \NN_+$ is the depth of the composition mapping. 
Here we set $\cX^L = \cY^L$ for ease of presentation. 
We aim to learn a target mapping in the class $\cF^*$, which captures the ground truth in a range of machine learning tasks \citep{vaswani2017attention, dosovitskiy2020image, bloem2020probabilistic}.
As shown in \cite{bloem2020probabilistic}, any equivariant mapping admits the following reparameterization,
\begin{align}\label{eq:equiv-f}
	[F_t(X)]^\ell = f(X^\ell, \hat \PP_X),
\end{align}
where $f: \cX \times \cP(\cX) \rightarrow \cY$ is a measurable function, $X = (x^1, \ldots, x^L) \in \cX^L$ is a sequence, $\hat \PP_X = L^{-1} \sum_{j = 1}^L \delta_{x^\ell}$ is its empirical distribution. Here we denote by $[F_t(X)]^\ell$ the $j$-th component $F_t(X) = ([F_t(X)]^1, [F_t(X)]^2, \ldots, [F_t(X)]^L) \in \cY^L$.

%The following proposition characterizes the reparameterization properties of equivariant mappings. Here we consider $X = (x^1, \ldots, x^L) \in \cX^L$ to be a sequence and denote by $\hat \PP_X = L^{-1} \sum_{j = 1}^L \delta_{x^\ell}$ its empirical distribution.
%
%\begin{proposition}[Reparameterization of Equivariant Mapping \citep{bloem2020probabilistic}]
%	\label{prop:inv-eqv}
%	Let $X \in \cX^L$ be a random sequences and $F: \cX^L \rightarrow \cY^L$ be a sequence to sequence mapping. We assume $[F(X)]^\ell$ is independent to $[F(X)]^i,\ i \neq j$ when conditioned on $X$. Then, the mapping $F$ is equivariant if and only if there is a function $f: \cX \times \cP(\cX) \rightarrow \cY$ such that
%	\begin{align}\label{eq:equiv-f}
%		[F(X)]^\ell = f(X^\ell, \hat \PP_X).
%	\end{align}
%\end{proposition}

The transformer \citep{vaswani2017attention, dosovitskiy2020image} aims to parameterize the mapping in the class $\cF^*$ defined in \eqref{eq:fc-tar} by the composition of transformer encoders. Specifically, we define the following class of transformers,
\begin{align}
	\label{eq:trans}
	\cF_\Theta^L = \bigl\{ \underbrace{\enc \circ \enc \circ \cdots \enc}_{T ~\enc \mathrm{s}}(\cdot; \theta) : \cX^L \rightarrow \cX^L \biggiven \theta = (\theta^{(0)}, \ldots \theta^{(T-1)}) \in \Theta^T \bigr\}.
\end{align}
Here $\theta$ is the (learnable) parameter and the $t$-th transformer encoder with the parameter $\theta^{(t)}$ takes the following form,
\begin{align}
	\label{eq:encoder0}
	X^{(t + 1)} = \enc(X^{(t)}; \theta^{(t)}) = \nn \circ \mha (X^{(t)}; \theta^{(t)}),
\end{align}
where $X^{(t)}$ is the output of the $(t-1)$-th transformer encoder when $t \ge 1$ and the input sequence $X$ when $t = 0$, $\mha$ is the multi-head self-attention defined in \eqref{eq:mha} subsequently, and $\nn$ denotes the composition of multi-layer perceptrons (MLP), residual connections, and layer normalizations specified subsequently. Here $\theta^{(t)}$ is the (learnable) parameter in the $t$-th transformer encoder. 
Also, the input sequence $X$ includes the positional embedding, which allows us to cast it as an unordered set.
In the following section, we show that $\mha$ is equivariant. Since $\nn$ is position-wise, it preserves the equivariance of $\mha$. Thus, the transformer encoder is equivariant, which allows us  to exploit the equivariance of the target mapping in $\cF^*$ in \eqref{eq:fc-tar}.
%By \eqref{eq:equiv-f}, the transformer encoder has the following form,
%\begin{align}
%	\label{eq:repara}
%	z_{t+1}^\ell = f(z_{t}^\ell, \hat \PP_{Z_t}),
%\end{align}
%where $f: \cX \times \cP(\cX) \rightarrow \cY$ is a measurable function. Moreover, as the length $L$ of the input tends to infinity, the empirical distribution $\hat \PP_{Z_t}$ converges to the population distribution $\PP_{Z_t}$. Thus, the transformer encoder mapping approximates $f(\cdot , \PP_{Z_t})$ as $L \rightarrow \infty$, which allows us to handle long sequences.

\subsection{Attention Approximates Conditional Mean Embedding} \label{sec:attn}
In what follows, we characterize the multi-head self-attention $\mha$ in a transformer encoder $\enc$, which is a layer of the transformer as specified in \eqref{eq:trans}. 
Given a sequence $X \in \RR^{L\times d}$, which is the input sequence of the transformer or the output sequence of the previous layer, we compute the query $Q\in \RR^{L\times d_\tp}$, key $K \in \RR^{L\times d_\tp}$, and value $V \in \RR^{L\times d}$ via
\begin{align}\label{eq:qkvw}
	Q = X W^\tq, \quad K = X W^\tk, \quad V = XW^\tv,
\end{align}
where $W^\tq, W^\tv \in \RR^{d\times d_\tp}$ and $W^\tv \in \RR^{d \times d}$ are the (learnable) parameters. For ease of presentation, we denote by $q^\ell$, $k^\ell$, and $v^\ell$ the $\ell$-th row of $Q$, $K$, and $V$, respectively.  
%TODO verify this: and assume that $(q^\ell, k^\ell, v^\ell)$ are samples from $\PP_{(Q, K, V)}$.  We assumes that $\max_\ell\{\norm{q^\ell}, \norm{k^\ell}, \norm{v^\ell}\} \le 1$, which can be achieved via normalization.
%We are given the query $Q \in \RR^{L \times d_k}$, key $K \in \RR^{L \times d_k}$, and value $V \in \RR^{L \times d_v}$, which are sequences of length $L$ and take the form of $G = (g^1, g^2, \ldots, g^L) ^\top $ for $g = q, k, v$. Note that the dimensions of query and the key are the same since they come from the same space. We denote the joint distribution of $(k^\ell, v^\ell)$ by $\PP_{(K, V)}$. Moreover, we assume that $\max_\ell\{\norm{q^\ell}, \norm{k^\ell}, \norm{v^\ell}\} \le 1$ and denote by $\cK$ and $\cV$ the spaces of key and value, respectively. Such bounded queries, keys, and values can be attained via appropriate normalization. The entire dataset takes the form of $\cD = \{(Q_i, K_i, V_i)\}_{i = 1}^n$, where $Q_i$, $K_i$, and $V_i$ are the query, key, and value calculated from the $i$-th input sequence $X_i \in \RR^{L\times d}$. Specifically, in self-attention, query, key, and value are calculated via
%\begin{align*}
%	Q = X W^\tq, \quad K = X W^\tk, \quad V = XW^\tv,
%\end{align*}
%where $W^\tq, W^\tv \in \RR^{d\times d_k}$ and $W^\tv \in \RR^{d \times d_v}$, and $X$ is either the input sequence or the output from the previous neural network layers.
%For notational simplicity, we omit the subscription $i$ that denotes the $i$-th sequence.
To define the multi-head self-attention $\mha$ in \eqref{eq:encoder0}, we define the attention as follows
\begin{align} \label{eq:trfm}
	\att(Q, K, V) & =  \Norm\bigl(\fk(Q, K) \bigr) V \in \RR^{L\times d}
\end{align}
for any $Q, K \in \RR^{L\times d_\tp}$ and $V \in \RR^{L\times d}$.
where $\fk(Q, K) = (\fk(q^i, k^\ell))_{i, j \in [L]}$ is a matrix for a kernel $\fk: \RR^{d_\tp} \times \RR^{d_\tp} \rightarrow \RR$ and $\Norm: \RR^{L\times L} \rightarrow \RR^{L\times L}$ is an operator that normalizes $\fk(Q, K)$. 
Specifically, in the dot-product attention \citep{vaswani2017attention}, we have
\begin{align}
	\label{eq:dotp-attn}
	\fk(q, k) = \exp(q^\top k), \qquad \Norm(A) = \diag( A \mathbf{1}_L )^{-1} A \in \RR^{L \times L}
\end{align}
for any $A \in \RR^{L\times L}$.
Here $\mathbf{1}_L$ is the all-one vector in $\RR^L$.
Let $q \in \RR^{d_\tp}$ be a row of  $Q$. The corresponding row of $\att(Q, K, V)$ takes the following form,
\begin{align}\label{eq:attq}
	\att(q, K, V) & = V^\top \Norm\bigl(\fk(K, q) \bigr) \in \RR^{d},
\end{align}
where $\fk(K, q) = (\fk(k^\ell, q))_{j \in [L]} \in \RR^{L}$. Based on the definition of the attention $\att$ in \eqref{eq:trfm}, we define the multi-head self-attention $\mha$ in \eqref{eq:encoder0} as
\begin{align}\label{eq:mha}
	\mha(X; w) = \sum_{i= 1}^h \head_i \in \RR^{L\times d}.
\end{align}
Here $h\in \NN_+$ is the number of heads, $w = \{(W_i^\tq, W_i^\tk, W_i^\tv)\}_{i = 1}^h$ is the (learnable) parameter, and
\begin{align}\label{eq:mha-head}
	\head_i = \att(Q_i, K_i, V_i) \in \RR^{L\times d}, \qquad Q_i = X W_i^\tq, \quad K_i = X W_i^\tk, \quad V = XW_i^\tv.
\end{align}
We remark that such a definition of the multi-head self-attention in \eqref{eq:mha} is equivalent to that in \cite{vaswani2017attention}, which is illustrated in \S\ref{sec:equiv}.

Since the input sequence $X\in \RR^{L\times d}$ includes the positional embeddings, the rows $\{x^\ell\}_{\ell \in [L]}$ are exchangeable across the indices $\ell \in [L]$. 
Thus, by the definition of $Q$, $K$, and $V$ in \eqref{eq:qkvw}, the rows $\{(q^\ell, k^\ell, v^\ell)\}_{\ell \in [L]}$ are also exchangeable. 
We denote by $\hat \PP_{(Q, K, V)} = L^{-1} \sum_{\ell = 1}^{L} \delta_{(q^\ell, k^\ell, v^\ell)}$ the empirical distribution of $\{(q^\ell, k^\ell, v^\ell)\}_{\ell \in [L]}$. 
Correspondingly, let $\PP_{(Q, K, V)}$ be the population distribution, which corresponds to $L \rightarrow \infty$.
In \eqref{eq:trfm}, we consider the following normalization,
\begin{align}
	\label{eq:norm-cme}
	\Norm\bigl(\fk(Q, K) \bigr) = \fk(Q, K)\bigl(\fk(K, K) + L\lambda I_L\bigr)^{-1},
\end{align}
where $\fk(K, K) = (\fk(k^i, k^\ell))_{i, j \in [L]} \in \RR^{L\times L}$ is the Gram matrix, $L \in \NN_+$ is the sequence length, and $\lambda > 0$ is the regularization parameter. We consider the RKHS $\cH_k$ and $\RR^d$ (as a finite-dimensional RKHS) with the kernels $\fk(\cdot, \cdot)$ and $\inp{\cdot}{\cdot}$, respectively. Here $\inp{\cdot}{\cdot}$ is the Euclidean kernel. 
See \S\ref{sec:attn-model-ortho} for a detailed discussion on the efficient implementation of the normalization in \eqref{eq:norm-cme} and its practical implication.

Let $\cC_{KK}$ be the covariance operator defined in \eqref{eq:cov} for the marginal distribution $\PP_K$ of $\PP_{(Q, K, V)}$ with respect to $K$.  
The following theorem characterizes the error of approximating conditional mean embedding by the attention.

%{\red STOP HERE}
%
%Recall that the joint distribution of the rows of $K$ and $V$ is $\PP_{(K, V)}$. We consider the RKHS $\cH_k$ and $\cH_v$ with kernels $\fk$ and $\fl$. In what follows, we show that the attention mapping in \eqref{eq:trfm} approximates the conditional mean embedding $\cme(q, \PP_{(K, V)})$. 
%Recall from \eqref{eq:reg-int-emp2} that the conditional mean embedding can be approximated via
%\begin{align}
%	\label{eq:cme}
%	\hat \cme_\lambda(q, \PP_{(K, V)}) =  V^\top (\fk(K, K) + L\lambda I_L)^{-1} \fk(K, q) = V^\top \Norm\bigl(\fk(K, q) \bigr),
%\end{align}
%which can be viewed as an attention mapping in \eqref{eq:trfm} by taking the matrix inverse as a normalization operator.
%%In particular, the conditional mean embedding takes the following form,
%%\begin{align}\label{eq:cme-qkv}
%%	\cme(q, \PP_{(K, V)}) = \EE_{\PP_{(K, V)}}[ v \biggiven k = q ] = \cC_{V\given K} \fk(q, \cdot).
%%\end{align}
%We consider that $\cH_v$ is the dual space of $\cV$ and equipped with the Euclidean kernel $\fl(v, v') = \inp{v}{v'}$. 
%The following Theorem characterizes the approximation error of the empirical conditional mean embedding,


\begin{theorem}[Attention Approximates Conditional Mean Embedding]
	\label{prop:attn-cme}
	We assume that the kernel $\fk$ is positive definite and $\fk(q, \cdot)$ is in the range of $\cC_{KK}$ for any $q \in \RR^{d_\tp}$. 
	Let the normalization in the attention take the form in \eqref{eq:norm-cme}. Then, the attention recovers the empirical conditional mean embedding defined in \eqref{eq:reg-int-emp2}.
	Moreover, it holds with probability at least $1-\delta$ that for any $q \in \RR^{d_\tp}$,
	\begin{align*}
		\norm[\big]{\att(q, K, V) - \cme(q, \PP_{(K, V)})}_2 = \cO\bigl((L^{-1} + \sqrt{\Tr(\cC_{KK})/ L})\log(1/\delta) + \lambda\bigr),
	\end{align*}
 	where $\PP_{(K, V)}$ is the marginal distribution of $\PP_{(Q, K, V)}$ with respect to $(K, V)$ and $ \Tr(\cC_{KK})$ is the trace of $\cC_{KK}$.
\end{theorem}

\begin{proof}
	%TODO Complete the proof
	See \S\ref{sec:pf-thm-attn-cme} for a detailed proof.
\end{proof}

We highlight the following implications of Theorem \ref{prop:attn-cme}.
%\subsection{Attention Approximates Conditional Mean Embedding}
%In what follows, we show that attention parameterizes the conditional mean embedding.
%Recall that $\cC_{V\given K}^\lambda$ denotes regularized conditional mean embedding operator solves the least squares problem in \eqref{eq:reg-int}. Correspondingly, we define the regularized conditional mean embedding as
%\begin{align}\label{eq:cme-reg}
%	\cme_\lambda(q, \PP_{(K, V)})  = \cC_{V\given K}^\lambda \fk(q, \cdot),
%\end{align}
%where $\lambda > 0$ is the regularization parameter. In what follows, we show that the without the normalization operator, the following attention mapping
%\begin{align}\label{eq:att-unorm}
%	\att(q, K, V) & = V^\top\fk(K, q) ,
%\end{align}
%approximates the regularized conditional mean embedding. We first impose the following assumption on the kernel $\fk(\cdot, \cdot)$.
%
%\begin{assumption}\label{asp:attn-cme}
%	We make the following assumptions on the kernel.
%	\begin{itemize}
%		\item[(i).] The kernel $\fk(\cdot, \cdot)$ is positive definite and satisfies that $\max_{k \in \cK} \fk(k, k) < 1/2$.
%		\item[(ii).] The rows $\{(k^i, v^i)\}_{i \in [L]}$ of $(K, V)$ are i.i.d.\ samples from the joint distribution $\PP_{(K, V)}$.
%	\end{itemize}
%\end{assumption}
%Assumption \ref{asp:attn-cme} (i) can be achieved via normalization. We remark that this assumption is needed for the ease of presentation and can be relaxed to $\fk(k, k) \le r$ for any $r < 1$. Here for the ease of presentation, we consider $r = 1/2$.
%
%The following theorem characterizes the approximation of the regularized conditional mean embedding via the attention mapping.
%
%\begin{theorem}[Attention Approximates Regularized Conditional Mean Embedding]
%	\label{thm:attn-cme}
%	Under Assumption \ref{asp:attn-cme}, the attention mapping in \eqref{eq:att-unorm} approximates the regularized conditional mean embedding $\cme_\lambda$ for $\lambda > 0$ and RKHS $\tilde \cH$ with kernel $\tilde \fk(\cdot, \cdot)$. Specifically, it holds with probability at least $1 - \delta$ that
%	\begin{align*}
%		\max_{q\in \cK} \norm[\big]{\att(q, K, V) - \cme_\lambda(q, \PP_{(K, V)})} \le 2\biggl( \frac{2}{L} + \sqrt{\frac{\Tr(\cC_{KK})}{L}} \biggr) \cdot\log\frac{2}{\delta},
%	\end{align*}
%	where $\Tr(\cC_{KK})$ is the trace of the covariance operator $\cC_{KK}$ and  $L$ is the length of the sequence and $\cC_{KK}$ is the covariance operator.
%\end{theorem}
%\begin{proof}
%	See \S\ref{sec:pf-thm-attn-cme} for a detailed proof.
%\end{proof}
%
%\vspace{4pt}

\noindent{\bf What class does transformer approximate?}
The reparameterization in \eqref{eq:equiv-f} allows us to represent an equivariant mapping in the form of $f: \RR^d \times \cP(\RR^d) \rightarrow \RR^d$. 
In what follows, we view the transformer from such an aspect. 
Let the space of input sequences be $\cX^L = \RR^{L\times d}$ in \eqref{eq:trans}.
Note that the input sequence $X \in \RR^{L \times d}$ of the transformer is exchangeable across the indices $\ell \in [L]$. 
Thus, since it includes the positional embedding, the input sequence is represented by its empirical distribution $\hat \PP_X$, which converges to the population distribution $\PP_X$. 
Also, Theorem \ref{prop:attn-cme} shows that the attention converges to the conditional mean embedding as $L\rightarrow \infty$.
In what follows, we consider the class of transformers with $L\rightarrow \infty$. 
We define the following class, which corresponds to the entry-wise mappings of transformer,
\begin{align} \label{eq:fc-inf}
	\cG_\Theta = \bigl\{ \underbrace{\ence \circ \ence \circ \cdots \ence}_{T ~\ence\mathrm{s}}(\cdot; \theta) :\RR^d \times \cP(\RR^d) \rightarrow \RR^d \biggiven \theta = (\theta^{(0)}, \ldots, \theta^{(T-1)}) \in \Theta^T \bigr\}.
\end{align}
Here the $t$-th $\ence $ takes the following form,
\begin{align*}
	x^{(t+1)} = \ence(x^{(t)}; \PP_{X^{(t)}}, \theta^{(t)}) = \nn\Bigl(\sum_{i=1}^{h}\cme(q^{(t)}_i, \PP_{(K_i^{(t)}, V_i^{(t)})}); \theta^{(t)} \Bigr),
\end{align*}
where $h$ is the number of heads, $\theta^{(t)} \in \Theta$ is the parameter, and
\begin{align*}
	q^{(t)}_i = (W^{\tq, (t)}_i)^\top x^{(t)}, \qquad \PP_{(K_i^{(t)}, V_i^{(t)})} = \bigl((W_i^{\tk, (t)})^\top, (W_i^{\tv, (t)})^\top \bigr)_\sharp  \PP_{X^{(t)}}.
\end{align*}
Moreover, $\PP_{X^{(t + 1)}}$ is the following pushforward distribution of $\PP_{X^{(t)}}$,
\begin{align}
	\PP_{X^{(t + 1)}} = \bigl(\ence(\cdot; \PP_{X^{(t)}}, \theta^{(t)})\bigr)_\sharp \PP_{X^{(t)}}.
\end{align}
In particular, the input is $x^{(0)} = x$ and $\PP_{X^{(0)}} = \PP_X$. 
Recall the definition of the class $\cF_\Theta^L$ of transformers in \eqref{eq:trans}. Let $X \in \RR^{L\times d}$ be a sequence whose rows are sampled from $\PP_X$. 
Then, for any transformer $F \in \cF_\Theta^L$, Theorem \ref{prop:attn-cme} shows that 
\begin{align} \label{eq:approx-linf}
	[F(X; \theta)]^\ell \rightarrow f(x^\ell, \PP_X; \theta) \in \cG_\Theta
\end{align}
as $L\rightarrow \infty$ for any $j \in [L]$. Here $x^\ell$ and $ [F(X; \theta)]^\ell$ are the $j$-th rows of $X$ and $F(X; \theta)$, respectively. 

Note that $\cG_\Theta$ defines the entry-wise mapping for the given population distribution $\PP_X$. In what follows, we turns to the seq2seq mapping when $L \rightarrow \infty$.
Corresponding to the class of functions from $\RR^{L\times d}$, we define the following function class for any index set $\cL$, whose carnality $|\cL|$ can be infinite, 
\begin{align}
	\label{eq:fcfi}
	\cF_\Theta^\cL = \bigl\{ \bar F: (\RR^d)^\cL \rightarrow (\RR^d)^\cL \biggiven [\bar F(X; \theta)]^\ell = f(x^\ell, \PP_X; \theta), \forall \ell \in \cL, f \in \cG_\Theta^\infty  \bigr\}.
\end{align}
Here $\PP_X$ denotes the population distribution of $X\in (\RR^d)^\cL$. 
Recall that $\cF_\Theta^L$ is the class of the transformers defined in \eqref{eq:trans}.
Note that when $L \le L'$, we can view the relation between $\cF_\Theta^L$ and $\cF_\Theta^{L'}$ as $\cF_\Theta^L \subseteq \cF_\Theta^{L'}$, since we can truncate a mapping of $\cX^{L'} \rightarrow \cX^{L'}$ to $\cX^{L} \rightarrow \cX^{L}$.
Then, the convergence in \eqref{eq:approx-linf} is illustrated as the following approximation between classes of mappings, 
\begin{align}\label{eq:approx-fc}
	\cF_\Theta^L \rightarrow \cF_\Theta^\infty:
\end{align}
as $L \rightarrow \infty$. Here $\cF_\Theta^\infty=\cF_\Theta^\cL$, where $\cL = \NN_+$ is the limit of $[L] = \{1, 2, \ldots, L\}$ as $L\rightarrow \infty$. 
{\red  and the convergence is in the sense that $\cup_{L = 1}^\infty \cF_\Theta^L = \cF_\Theta^\infty$.} 
We illustrate the relation among $\cF_\Theta^L$, $\cF_\Theta^\infty$, and class of equivariant mappings in Figure \ref{fig:fc}.

We remark that transformer allows different sequence lengths $L$ by exploiting the equivariance.
And the transformers with different sequence lengths $L$ approximates the same class of seq2seq mappings when $L\rightarrow \infty$.
In particular, the attention of the transformer encoder approximates the conditional mean embedding when $L\rightarrow \infty$, which exploits the interaction among entries of the sequence and captures relational reasoning.



\begin{figure}
	\label{fig:fc}
	\centering
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.7,xscale=0.7]
	%uncomment if require: \path (0,780); %set diagram left start at 0, and has height of 780
	
	%Flowchart: Connector [id:dp1752030377917666] 
	\draw   (88,336.58) .. controls (88,253.42) and (207.76,186) .. (355.5,186) .. controls (503.24,186) and (623,253.42) .. (623,336.58) .. controls (623,419.75) and (503.24,487.17) .. (355.5,487.17) .. controls (207.76,487.17) and (88,419.75) .. (88,336.58) -- cycle ;
	%Flowchart: Connector [id:dp7942325895336104] 
	\draw   (157,336.54) .. controls (157,302.81) and (192.82,275.46) .. (237,275.46) .. controls (281.18,275.46) and (317,302.81) .. (317,336.54) .. controls (317,370.28) and (281.18,397.62) .. (237,397.62) .. controls (192.82,397.62) and (157,370.28) .. (157,336.54) -- cycle ;
	%Straight Lines [id:da1546563591971537] 
	\draw    (317,336.54) -- (392,336.62) ;
	\draw [shift={(394,336.62)}, rotate = 180.06] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Flowchart: Connector [id:dp7634356750378293] 
	\draw   (394,336.62) .. controls (394,302.89) and (429.82,275.54) .. (474,275.54) .. controls (518.18,275.54) and (554,302.89) .. (554,336.62) .. controls (554,370.36) and (518.18,397.71) .. (474,397.71) .. controls (429.82,397.71) and (394,370.36) .. (394,336.62) -- cycle ;
	
	% Text Node
	\draw (349.5,217.58) node   [align=left] {\begin{minipage}[lt]{104.04pt}\setlength\topsep{0pt}
			Equivariant Mappings
	\end{minipage}};
	% Text Node
	\draw (234,340.08) node   [align=left] {\begin{minipage}[lt]{35.7pt}\setlength\topsep{0pt}
			\begin{center}
				$\displaystyle \mathcal{F}_{\Theta }^{L}$
			\end{center}
			
	\end{minipage}};
	% Text Node
	\draw (474,336.62) node   [align=left] {\begin{minipage}[lt]{23.12pt}\setlength\topsep{0pt}
			$\displaystyle \mathcal{F}_{\Theta }^{\infty }$
	\end{minipage}};
	% Text Node
	\draw (353.5,323.58) node   [align=left] {\begin{minipage}[lt]{38.76pt}\setlength\topsep{0pt}
			$\displaystyle L\rightarrow \infty $
	\end{minipage}};
	
	
\end{tikzpicture}
 \caption{Relation among $\cF_\Theta^L$, $\cF_\Theta^\infty$, and class of equivariant mappings}
\end{figure}


%{\red STOP HERE}
%
%By \eqref{eq:equiv-f}, letting $x = X^\ell \in \RR^d$, the corresponding $j$-th entry of the output of the $t$-th layer of the target mapping takes the form of
%\begin{align*}
%	[F_t(X)]^\ell = f(x, \hat \PP_X)
%\end{align*}
%for a function $f: \RR^d \times \cP(\RR^d) \rightarrow \RR^d$. 
%In what follows, we call $f$ the entry-wise mapping.
%When the sequence length $L \rightarrow \infty$, the entry-wise mapping approximates $f(x, \PP_X)$, where $\PP_X$ is the population distribution of $X$. In what follows, we show how the transformer encoder approximates the limiting mapping.
%
%Recall from \eqref{eq:encoder0} that a transformer encoder is the composition of $\nn$ and $\mha$, where by definition in \eqref{eq:mha} $\mha$ is the sum of multiple attentions. Specifically, the transformer encoder takes the following form,
%
%
%By Theorem \ref{prop:attn-cme} and the definition of conditional mean embedding in \eqref{eq:cme-opt}, it holds that
%\begin{align*}
%	\att(q, K, V) \rightarrow \EE_{\PP_{V\given K} }[v \given k = q ].
%\end{align*}
%By \eqref{eq:equiv-f}, the entry of equivariant mapping takes the form of $g(x, \hat \PP_X)$, which converges to $g(x, \PP_X)$ as the sequence length $L\rightarrow \infty$. In what follows, we show how attention parameterizes the function $g(x, \PP_X)$. Note that $g$ is a function of the entry $x$ and the distribution $\PP_X$. We illustrate the computational graph of $g$ with respect to $x$ and $\PP_X$ for $i \in [h]$ as follows,
%\begin{align}
%	\label{eq:pip}
%	x &\xrightarrow{(W_i^\tq)^\top } q_i, \noend
%	\PP_{X} &\xrightarrow{(W_i^\tk, W_i^\tv)_{\sharp}} \PP_{(K_i, V_i)} \xrightarrow{\text{attention}} \EE_{\PP_{V_i\given K_i} }[v \given k = \cdot ].
%\end{align}
%Then, the function $g$ takes the form of
%\begin{align*}
%	g(x, \PP_X) = \nn \Bigl(\sum_{i = 1}^{h}\EE_{\PP_{V_i\given K_i} }[v \given k = q_i ]\Bigr).
%\end{align*}
%




%Without any normalization in the attention mapping \eqref{eq:attq}, it holds that
%\begin{align}\label{eq:ckv}
%	L^{-1} \att(q, K, V) =  L^{-1}V^\top \fk(K, q) \rightarrow \cC_{VK} \fk(q, \cdot),
%\end{align}
%where $\cC_{VK}$ is the covariance operator. We remark that such an approximation shows that the attention mapping is a variational autoencoder for the probability distribution.
%According to \eqref{eq:equiv-f}, to parameterize an equivariant mapping, we need to parameterize the probability distribution $\PP_X$. However, the probability distribution $\PP_X$ is infinite-dimensional, and thus, there is a gap to parameterize its function by finite-dimensional parameters. Recall from \eqref{eq:qkvw} that the query $Q$, key $K$, and value $V$ are calculated via low-rank linear mapping when $d_\tp < d$. We illustrate such a variational autoencoder (VAE) as follows,
%\begin{align}
%	\label{eq:pip2}
%	\PP_{X} \xrightarrow{(W^\tk, W^\tv)_{\sharp}} \PP_{(K, V)} \xrightarrow{\text{attention}} \cC_{VK}.
%\end{align}
%The low-rankness of such a VAE comes from two aspects. Firstly, the parameter $W^\tk\in \RR^{d\times d_\tp}$ is low-rank since $d_\tp < d$. Note that in the multi-head self-attentions with $h$ heads, it holds that $d_\tp h = d$, which allows to recover from the low-rank representation.
%Second, the expressive power of the covariance operator depends on the kernel $\fk$ and $\fl$. Recall that we consider $\fl$ as the Euclidean inner product, which is finite-dimensional. Thus, such a covariance operator serves as a low-rank representation of $\PP_{(K, V)}$.

%TODO {To illustrate what such a VAE infers, we consider the effect of the normalization.}

\vspace{4pt}

%\noindent{\bf The gap from the regularization.}
%Without additional assumptions, the gap between $\cme_\lambda$ and $\cme$ may not vanish as $\lambda $ goes to zero, as the construction of the RKHS $(\tilde \cH, \tilde \fk)$ for the conditional mean embedding depends on the regularization parameter $\lambda > 0$.  We note that such a gap is due to the lack of an explicit inverse in the attention mapping. Specifically, when we consider the fixed kernel $\fk(\cdot, \cdot)$, \cite{song2009hilbert} shows that the conditional mean embedding can be approximated consistently via
%\begin{align*}
%	\fk(Q, K) \bigl(\fk(K, K) + L\lambda \cdot I_L \bigr)^{-1} V,
%\end{align*}
%which normalizes the mapping via a $L \times L$ matrix inverse $(\fk(K, K) + L\lambda \cdot I_L )^{-1}$.
%In comparison, the attention mapping in \eqref{eq:trfm} normalizes the mapping via the inverse of the diagonal matrix $D = \diag(\sigma^1, \ldots, \sigma^L)$. We remark that the gap between $\cme_\lambda$ and $\cme$ comes from the difference of the normalization.
%
%\vspace{4pt}

\noindent{\bf Necessity of the multiple heads.}
We remark that Theorem \ref{prop:attn-cme} shows the necessity of the multiple heads in $\mha$. 
Recall from \eqref{eq:qkvw} that the query $Q \in \RR^{L \times d_\tp}$, key $K \in \RR^{L\times d_\tp}$, and $V \in \RR^{L\times d}$ at a head linear transformations of the input sequence $ X \in \RR^{L \times d}$. 
In multi-head self-attentions \citep{vaswani2017attention}, it is set that $d = d_\tp \cdot h$, where $h$ is the number of heads. In single-head self-attentions, where $h=1$ and $d_\tp = d$, the matrices $W^\tq, W^\tk, W^\tv \in \RR^{d \times d}$ may be invertible, in which case the attention approximates the following conditional mean embedding,
\begin{align*}
	\cme(q, \PP_{(K, V)}) = \EE_{\PP_X}[ (W^\tv)^\top x \given (W^\tk)^\top x = q ] = \bigl((W^\tk)^{-1} W^\tv \bigr)^\top q = \bigl(W^\tq (W^\tk)^{-1} W^\tv \bigr)^\top x,
\end{align*}
which is a linear mapping and fails to parameterize the interactions between different entries $x^{\ell_1}$ and $x^{\ell_2}$.
In comparison, in the case where $d_\tp < d$, the matrices $W^\tq, W^\tk \in \RR^{d \times d_\tp}$ are not invertible and thus, the conditional mean embedding is a nonlinear mapping. 
Thus, to add nonlinearity to the attention, it is necessary to set multiple heads, where $h > 1$ and $d_\tp < d$.
%In particular, the structure of multi-head attention is as follows,
%\begin{align}\label{eq:mha}
%	\mha(Q, K, V) = [\head_1; \ldots ; \head_h] W^o,
%\end{align}
%where
%\begin{align}\label{eq:mha-head}
%	\head_i = \att(Q_i, K_i, V_i).
%\end{align}
%Here $[;]$ is the concatenation operation, $Q_i, K_i, V_i \in \RR^{L\times d_\tp}$ for $i \in [h]$ are the queries, keys, and values at the $i$-th head, and $W^o \in \RR^{d_\tp h \times d}$ is the learnable parameter.
%
%{\red ======}
%
%By writing $W^o = ((W^o_1)^\top, \ldots, (W^o_h)^\top)^\top$ and
%\begin{align*}
%	\tilde\head_i = \head_i W^o_i,
%\end{align*}
%the multi-head attention in \eqref{eq:mha} is equivalent to the following
%\begin{align}\label{eq:mha1}
%	\mha(Q, K, V) = \sum_{i= 1}^h \tilde \head_i.
%\end{align}
%We remark that the concatenation form in \eqref{eq:mha} is preferred because it results in computationally efficient matrix multiplication \citep{bibid}. Here, we consider the equivalent additive form in \eqref{eq:mha} since it is better for theoretical analysis.
%
%{\red ==============}

\vspace{4pt}

%TODO IV
\noindent{\bf Instrumental variable.} 
The approximation of conditional mean embedding in Theorem \ref{prop:attn-cme} shows that attention is effective in causal inference. For the ease of presentation, we consider the following mapping,
\begin{align}
	\label{eq:iv}
	\nn \circ \att(Q, K, V) \in \RR^{L\times d},
\end{align}
which can be viewed as a simplified version of the transformer encoder. 
Here $\nn$ is a row-wise mapping. 
Let $q$ be a row of $Q$. 
By Theorem \ref{prop:attn-cme}, it holds that
\begin{align*}
	\att(q, K, V) \rightarrow \EE_{\PP_{V\given K}}[v \given k = q]
\end{align*}
as $L \rightarrow \infty$. 
Then, when $L \rightarrow \infty$, the mapping in \eqref{eq:iv} converges to 
\begin{align*}
	\nn \bigl(\EE_{\PP_{V\given K}}[v \given k = q]\bigr).
\end{align*}
Let the target output be $Y = (y^1, \ldots, y^L)^\top \in \RR^{L\times d}$. Note that $\nn$ is an universal function approximation with the (learnable) parameter $\theta$. Then, the learning problem can be formulated as maximizing the following log-likelihood takes the following form,
\begin{align*}
	\max_\theta \sum_{\ell = 1}^L \log \PP_\theta\bigl(y^\ell \biggiven \EE_{v \sim \PP_{V\given K = q^\ell}}[v] \bigr).
\end{align*}
Thus, the key $K$ can be viewed as the instrumental variable. Recall from \eqref{eq:qkvw}, the mapping from the input sequence $X$ to $Q$, $K$, and $V$ is learnable, which shows that transformer is effective in identifying the best instrumental variable. 


%\vspace{4pt}
%
%\noindent{\bf Equivariance and Invariance of multi-head Self-Attention.} We now show that the multi-head self-attention admits the form in \eqref{eq:equiv-f}. We see that the $W^o$ mapping is positional-wise. Thus, it suffices to show that any head admits the form of \eqref{eq:equiv-f}. By the mapping in \eqref{eq:qkv-sa}, we have that
%\begin{align*}
%	\hat \PP_{(K, V)} = \bigl((W^\tk)^\top, (W^\tv)^\top \bigr)_\sharp \hat \PP_X,
%\end{align*}
%where we denote by $((W^\tk)^\top, (W^\tv)^\top)_\sharp$ the pushforward mapping.
%We consider the feature mapping $\phi$ with respect to $\fk(\cdot, \cdot)$. Then, the attention mapping has the following form
%\begin{align*}
%	\att_*(q, K, V)  = L^{-1}\cdot V^\top \fk(K, q)  = \hat \cC_{VK}\fk(q, \cdot ).
%\end{align*}
%We also remark the above form inspires the design of attention mapping with linear computational complexity in the sequence length $L$ as in performer \citep{choromanski2020rethinking} and Galerkin transformer \citep{bibid}.



==> background.tex <==
%!TEX root = iclr2023_conference.tex

\section{Background} 

\noindent{\bf Reproducing kernel Hilbert space.} Let $\cH_x$ be a Hilbert space over a space $\cX$. We say $\cH_x$ is a reproducing kernel Hilbert space (RKHS) with kernel $\fk: \cX \times \cX \rightarrow \RR$ if it holds that
\begin{align}
	\label{eq:rkhs-ker}
	\inp[\big]{f}{\fk(x, \cdot)}_{\cH_x} = f(x), \quad \forall f \in \cH_x, x\in \cX.
\end{align}
Note that $\fk(x, \cdot)$ can be viewed as a feature mapping from $x \in \cX$ to $\cH_x$. Examples of the kernel include the polynomial kernel $\fk(x, x') = \inp{x}{x'}^d$ and the Gaussian radial basis function (RBF) kernel \#\label{eq:rbf}
\fk(x, x') = \exp(-\norm{x - x'}^2/2\sigma^2).
\#

\vspace{4pt}

\noindent{\bf Hilbert-Schmidt operator.}
Let $\cH_x$ and $\cH_y$ be two (separable) Hilbert spaces over spaces $\cX$ and $\cY$, and $(\phi_i)_{i \in I}$ and $(\psi_j)_{j \in J}$ be their orthonormal bases, respectively. The Hilbert-Schmidt norm of a (bounded) operator $\cC: \cH_x \rightarrow \cH_y$ is defined as
\begin{align}
	\label{eq:hs-norm}
	\norm{\cC}_\hs^2 = \sum_{i \in I, j \in J} \bigl| \inp{\cC \phi_i}{\psi_j}_{\cH_y} \bigr|^2.
\end{align}
A bounded operator $\cC: \cH_x \rightarrow \cH_y$ is a Hilbert-Schmidt operator if $\norm{\cC}_\hs < \infty$.

\vspace{4pt}

\noindent{\bf Conditional mean embedding.}
We first introduce conditional mean embedding, which embeds the conditional distribution to linear operators between RKHS. Let $\cH_x$ and $\cH_y$ be two RKHS over spaces $\cX$ and $\cY$ with kernel $\fk$ and $\fl$, respectively. Let $\PP_{(X, Y)}$ be the joint distribution of two random variables $X$ and $Y$ taking values in $\cX$ and $\cY$, respectively. The conditional mean embedding $\cme(x, \PP_{(X, Y)}) \in \cH_y$ of the conditional distribution $\PP_{Y \given x}$ is defined as 
\begin{align}
	\cme(x, \PP_{(X, Y)}) = \EE_{\PP_{(X, Y)}} \bigl[\fl(y, \cdot) \biggiven X= x\bigr].
\end{align}
Then, for any function $ g\in \cH_y$ and $x \in \cX$, it holds that
\begin{align*}
	\EE_{\PP_{(X, Y)}}\bigl[g(y) \biggiven X = x \bigr] = \inp{g}{\cme(x, \PP_{(X, Y)})}_{\cH_y}.
\end{align*}
The conditional mean embedding operator $\cC_{Y \given X}: \cH_x \rightarrow \cH_y$ is an operator that satisfies
\begin{align}
	\label{eq:cme-opt}
	\cC_{Y \given X} \fk(x, \cdot) = \cme(x, \PP_{(X, Y)}),
\end{align}
for any $x \in \cX$.
We define the (uncentered) covariance operator $\cC_{XX}: \cH_x \rightarrow \cH_x$ and the cross-covariance operator $\cC_{YX} : \cH_x \rightarrow \cH_y$ as follows, 
\begin{align}
	\label{eq:cov}
	\cC_{XX} = \EE_{\PP_X} \bigl[ \fk(x, \cdot) \otimes \fk(x, \cdot)\bigr], \quad \cC_{YX} = \EE_{\PP_{(X, Y)}} \bigl[ \fl(y, \cdot) \otimes \fk(x, \cdot)\bigr].
\end{align}
Here $\otimes$ is the tensor product. Then, it is shown that $\cC_{Y \given X} = \cC_{YX} \cC_{XX}^{-1}$ when $\cC_{Y \given X}$ exists \citep{song2009hilbert}. Moreover, we consider the following regularized least squares problem
	\begin{align}\label{eq:reg-int}
	\min_{\cC : \cH_x \rightarrow \cH_y}\cE_\lambda(\cC) = \EE_{\PP_{(X, Y)}} \Bigl[\norm[\big]{ \fl(y, \cdot) - \cC \fk(x, \cdot) }^2_{\cH_y} \Bigr] + \lambda \cdot \norm{\cC}^2_{\mathrm{HS}}, 
\end{align}
where $\norm{\cdot}_{\mathrm{HS}}$ denotes the Hilbert-Schmidt norm defined in \eqref{eq:hs-norm} and $\lambda > 0$ is the regularization parameter. The solution to \eqref{eq:reg-int} is given by $\cC^\lambda_{Y\given X} = \cC_{YX} (\cC_{XX} + \lambda)^{-1}$, which is interpreted as a regularized conditional mean embedding operator. Correspondingly, we consider the empirical least squares problem 
\begin{align}
	\label{eq:reg-int-emp}
	\hat \cE(\cU) =  \frac{1}{L}\sum_{\ell = 1}^{L} \norm[\big]{ \fl(y^\ell, \cdot) - \cC \fk(x^\ell, \cdot) }^2_{\cH_y} + \lambda \cdot \norm{\cC}^2_{\mathrm{HS}},
\end{align}
where $\{(x^\ell, y^\ell)\}_{\ell \in [L]}$ is a sample from $\PP_{(X, Y)}$. 
For the ease of presenting the solution to \eqref{eq:reg-int-emp}, we define the sampling operator $S_X: \cH_x \rightarrow \RR^L$ and $S_Y: \cH_y \rightarrow \RR^L$ as $S_X f = (f(x^1), \ldots, f(x^L))$ and $S_Y g = (g(y^1), \ldots, g(y^L))$ for $f \in \cH_x$ and $g \in \cH_y$, respectively. 
We denote by $S_X^*$ and $S_Y^*$ the adjoint of $S_X$ and $S_Y$, respectively.
We denote by $\hat \cC_{XX} = L^{-1} \sum_{\ell=1}^{L}\fk(x^\ell, \cdot) \otimes \fk(x^\ell, \cdot) = L^{-1}S_X^*S_X $ and $\hat \cC_{YX} = L^{-1} \sum_{\ell=1}^{L} \fl(y^\ell, \cdot) \otimes \fk(x^\ell, \cdot) = S_Y^*S_X$ the empirical (uncentered) covariance operator and (uncentered) cross-covariance operators, respectively.
Then, the solution to \eqref{eq:reg-int-emp} is given by $\hat \cC_{Y \given X}^\lambda = \hat \cC_{YX}(\hat \cC_{XX} + \lambda)^{-1}$. 
Moreover, following from the identity that $S_X(S_X^*S_X + L\lambda \cI)^{-1} = (S_XS_X^* + L \lambda I_L)^{-1} S_X$, it holds that
\begin{align}
	\label{eq:reg-int-emp2}
	\hat \cme_\lambda(x, \PP_{(X, Y)}) = \hat \cC_{Y \given X}^\lambda \fk(x, \cdot) = \hat \cC_{YX}(\hat \cC_{XX} + \lambda)^{-1} \fk(x, \cdot) = S_Y^* (\fk(X, X) + L\lambda I_L)^{-1} \fk(X, x).
\end{align}
Here $\fk(X, X) = S_xS_x^* = (\fk(x^i, x^j) )_{i, j \in [L]}$ is the Gram matrix and $\fk(X, x) = (\fk(x^1, x), \ldots, \fk(x^L, x))^\top$. 

\vskip4pt

\noindent{\bf Notations.}
Throughout this paper, we denote by lowercase letters (e.g., $x, y, q, k, v$) the rows of matrices or samples from distributions. We denote by uppercase letters (e.g., $X, Y, Q, K, V$) the corresponding matrices. 
We denote by $\delta_x$ the Dirac measure at a point $x$ over the space $\cX$, which satisfies that $\delta_x(A) = \ind \{x\in A\}$ for any subset $A \subseteq \cX$.
We denote by $[L]$ the set $\{1, 2, \ldots, L\}$ for any $L \in \NN_+$.
Given two measurable spaces $\cX$ and $\cY$, a mapping $f: \cX\rightarrow \cY$, and a probability distribution $\PP_X \in \cP(\cX)$, we denote by $f_\sharp \mu$ the pushforward distribution of $\mu$, which is given by
\begin{align}
	f_\sharp \PP_X(B) = \PP_X\bigl(f^{-1}(B)\bigr) 
\end{align}
for any measure subset $B \subseteq \cX$.

Let $r \geq 1$. We denote by $\|\cdot\|_r$ the typical vector $r$-norm. Also let $s \geq 1$, and $M = [m_1, \dots, m_{d_2}] \in \RR^{d_1\times d_2}$, where $m_i \in \RR^{d_1\times 1}$ for $i \in [d_2]$. We define the matrix $(r, s)$-norm as 
\$
\|M\|_{r, s} = \Bigl\|\bigl[\|m_1\|_r, \dots, \|m_{d_2}\|_r\bigr]\Bigr\|_s = \biggl(\sum_{i = 1}^{d_2}\|u_i\|^s_r\biggr)^{1/2}.
\$
We define the matrix operator norm $\|\cdot\|_{r \to s}$ as $\|M\|_{r\to s} = \sup_{u \in \RR^{d_2 \times 1}}\|Mu\|_{s}/\|u\|_r$. For positive reals $r$ and $s$ such that $1/r + 1/s = 1$, we call $(r, s)$ a conjugate pair.

%\begin{itemize}
%	\item Regression Interpretation
%
%	\item RKHS and Mercer's Theorem
%\end{itemize}
%
%RKHS: 
%spaces: $\cX, \cZ$, RKHS: $\cH, \fl$, kernels $\ker, g$, features $\phi, \varphi$
%\begin{align}
%	\ker(x, x') = \phi(x)^\top \phi(x'), \quad g(z, z') = \varphi(z) ^\top \varphi(z').
%\end{align}
%
%mean embedding
%\begin{align}
%	\mu_X = \EE[\phi(X)] = \EE[\ker(X, \cdot)] \in \RR^{d_\phi} = \cH_x
%\end{align}
%
%conditional mean embedding \citep{song2009hilbert}:
%\begin{align}\label{eq:cond_embedding}
%	\cU_{Y\given x} &= \EE_{(X, Y) \sim \PP}[\varphi(Y) \given X = x] \noend
%	& = \cC_{YX} \cC_{XX}^{-1} \ker(x, \cdot) 
%\end{align}
%Note that $\cU_{Y\given x} = \cU_{Y\given X} \ker(x, \cdot) = \cU_{Y \given X} \phi(x)$ and that for any $g \in \cH_y$ we have $\EE[g(Y) \given X = x] = \inp{g}{ \cU_{Y\given x}}$. We can view $\cU_{Y\given X}$ as an operator from $\cH_x$ to $\cH_y$. Furthermore, it holds that
%\begin{align}
%	\mu_Y = \cU_{Y \given X} \mu_X.
%\end{align}
%Thus, we can view the conditional mean embedding as a linear operator from $\cH_x$ to $\cH_y$. The conditional mean embedding can be approximated empirically as follows,
%\begin{align}
%	\label{eq:cond-emb-emp}
%	\hat \cU_{Y \given x} = \varphi(Y) \bigl(\phi(X)^\top \phi(X) + \lambda I_L \bigr)^{-1} \phi(X)^\top \phi(x) \in \RR^{d_\varphi} = \cH_y.
%\end{align}
%Moreover, the conditional mean embedding can be interpreted from the regression view. The conditional mean embedding $\cU_{Y\given X}$ is the minimizer of the following loss function for operator $\cU: \cH_x \rightarrow \cH_y$,
%
%
%
%
%Furthermore, the composition of the conditional mean embedding can be viewed as the product of the linear operators, i.e.,
%\begin{align} \label{eq:conditional_mean_embedding_composition}
%	\mu_Y = \cU_{Y \given X} \mu_X = \cU_{Y \given Z_L} \cU_{Z_{L - 1} \given Z_{L - 2}} \cdots \cU_{Z_2 \given Z_1} \cU_{Z_1 \given X} \mu_X.
%\end{align}
%Why composition?
%The relation in \eqref{eq:cond_embedding} holds under the condition that $\EE[g(Y)\given X = \cdot] \in \cH_x$ for $g \in \cH_y$. Thus, by composition, we improve the expressity of the operator.


\subsection{Reference}
PowerNorm \citep{shen2020powernorm}, Performer \citep{choromanski2020rethinking}, ViT \citep{dosovitskiy2020image}, Transformer \citep{vaswani2017attention}, invariance/equivariance \citep{bloem2020probabilistic}, conditional mean embedding \cite{song2009hilbert}

==> generalization.tex <==
%!TEX root = iclr2023_conference.tex

\section{Generalization: Breaking the Curse of Dimension}
In this section, we prove that the transformer generalizes regardless of the length $L$ of the input sequence.
\subsection{Transformer with Skip Connections}
We start by specifying the full structure of the transformer. In addition to the multihead self attention and FFN introduced in the previous sections, a transformer also adopts skip connections. We formally define the function class of $T$-layer transformer as follows. First, we define the multihead self attention with skip connection via
\$
Z^{(t)} = \mha(X^{(t)}W^q_t, X^{(t)}W^k_t, X^{(t)}W^v_t; W_t^o) + X^{(t)}.
\$
Then, without loss of generality, we define the typically used two-layer FFN (without bias terms), as 
\$
X^{(t+1)} = \nn(Z^{(t)}; A^z, A^\sigma) = \relu(Z^{(t)} A^z)A^\sigma + Z^{(t)}.
\$
where $A^z \in \RR^{d \times d_\sigma}, A^\sigma \in \RR^{d_\sigma \times d}$, and $\relu(\cdot)$ is the rectified linear unit (ReLU) that operates element-wise.


\vskip4pt
\noindent{\bf Function Class of Transformer.} To construct $\cF^\trans$, we start with the base case $\cF^A_0 = \{X^{(0)}\}$. Then we recursively define the function classes
\$
\cF_t^W & = \bigl\{\mha(X^{(t)}W^q_t, X^{(t)}W^k_t, X^{(t)}W^v_t; W_t^o)^\top + (X^{(t)})^\top: (W_t^q, W_t^k, W_t^v, W^o_t) \in {\cW}_t, X^{(t)} \in \cF_t^A\bigr\}, \\
\cF_{t+1}^A & = \bigl\{\nn(Z^{(t)}; A^z, A^\sigma)^\top: ({A}^z_t, A^\sigma_t) \in {\cA}_t, Z^{(t)} \in \cF_t^W\bigr\},
\$
where
\#
\cW_t & = \Bigl\{(W_t^{q}, W_t^{k}, W_t^{v}, W_t^o) \in \RR^{d \times d_k} \times\RR^{d \times d_k} \times\RR^{d \times d_p} \times\RR^{hd_p \times d}:\notag\\
& \quad\qquad \bigl\|(W_t^o)^\top\bigr\|_{r} \leq \omega^o_t, \bigl\|(W_t^o)^\top\bigr\|_{r, s} \leq R^o_t, \bigl\|(W_t^{q_i})^\top\bigr\|_{r} \leq \omega^{q_i}_t, \bigl\|(W_t^{k_i})^\top\bigr\|_{r} \leq \omega^{k_i}_t, \bigl\|(W_t^{v_i})^\top\bigr\|_{r} \leq \omega^{v_i}_t,\notag\\
& \quad\qquad \bigl\|(W_t^{q_i})^\top\bigr\|_{r, s} \leq R^{q_i}_t, \bigl\|(W_t^{k_i})^\top\bigr\|_{r, s} \leq R^{k_i}_t, \bigl\|(W_t^{v_i})^\top\bigr\|_{r, s} \leq R^{v_i}_t, \forall i \in [h]\Bigr\},\label{eq:set-wt}\\
{\cA}_t & = \Bigl\{(A_t^z, A_t^\sigma) \in \RR^{d \times d_\sigma} \times \RR^{d_\sigma \times d}:\notag\\
& \quad \qquad \bigl\|({A}_t^z)^\top\bigr\|_{r} \leq {\alpha}^z_t, \bigl\|({A}_t^z)^\top\bigr\|_{r, s} \leq {R}^z_t, \bigl\|({A}_t^\sigma)^\top\bigr\|_{r} \leq {\alpha}^\sigma_t, \bigl\|({A}_t^\sigma)^\top\bigr\|_{r, s} \leq R^\sigma_t \Bigr\},\label{eq:set-at}
\#
are the feasible parameter sets at the $t$-th composite layer. For a $T$-layer transformer, we have $\cF^\trans = \{ \agg \circ  f : f \in \cF^A_T\}$.


For ease of presentation, we define for $t \leq T-1$,
\#\label{eq:sum-head}
R_t^v = \sum_{i = 1}^hR_t^{v_i},\quad {\omega}_t^v = \sum_{i = 1}^h\omega_t^{v_i}, \quad \overline{\omega}_t^{qk} = \max_{i \in [h]} \{\omega_t^{q_i} + \omega_t^{k_i}\}, \quad {R}_t^{qk} = \sum_{i = 1}^h(R_t^{q_i} + R_t^{k_i})
\#
Then we write
\$
\tilde{\alpha}_t = 1 + \alpha_t^z \alpha_t^\sigma, \quad \tilde{\omega}_t^{vo} = 1 + \omega_t^o \omega_t^v
\$

\begin{theorem}[Transformer Generalization Error]\label{thm:gen}
Let $\cF_{\text{trans}}$ be a family of functions mapping from $\cD$ to $[0, 1]$. Then, for any $\delta > 0$, with probability at least $1 - \delta$ over the draw of an i.i.d. sample $\cD_n = \{(X_i, Y_i)\}_{i \in [n]}$ from the data distribution $\cD$, the following holds for all $f \in \cF_{\text{trans}}$,
\$
& \EE_{\cD}\Bigl[\ell\bigl(f(X), Y\bigr)\Bigr] - \hat{\EE}_{\cD_n}\Bigl[\ell\bigl(f(X), Y\bigr)\Bigr]\\
& \quad \leq 2 D \cdot \frac{2 + \sqrt{\log(1+R^\trans_T)} }{\sqrt{n}} + 3\sqrt{\frac{\log (2/\delta)}{n}},
\$
where $\hat{E}_{\cD_n}[\,\cdot\,]$ is the empirical mean over the sample $\cD_n$.
\end{theorem}


\vskip4pt
\noindent{\bf Near the Identity Layers.} Since the transformer adopts skip connections, we consider the case where each layer is close to the identity mapping.  

%\subsection{Lipschitz Continuous Conditional Mean Embedding Attention}
%We consider the empirical version of the conditional mean embedding
%\$
%\hat{\mathcal{U}}_{V\,|\, K = q} & = \hat{\cC}_{VK}(\hat{\cC}_{KK} + \lambda \cdot \cI)^{-1} \text{ker}(q,\cdot)\\
%& = \cS_V^* (\text{Ker}_K + L\lambda\cdot I_L)^{-1} \cS_K\text{ker}(q, \cdot).
%\$
%Here for any $\omega \in \RR^L$ and $f \in \cH_k$,
%\$
%\cS^*_V: \omega \to \omega^\top \Pi(V) = \sum_{l = 1}^L \omega_l \cdot \pi(v_l), \quad \cS_K : f \to (f(k_1), \dots, f(k_L))^\top.
%\$
%Alternatively, we can write the empirical conditional mean embedding as
%\$
%\hat{\mathcal{U}}_{V\,|\, K = q} = (\omega^{K, q})^{\top} \Pi(V), \quad \omega^{K, q} = (\text{Ker}_K + L\lambda\cdot I_L)^{-1} \cS_K \text{ker}(q, \cdot) \in \RR^{L\times 1}.
%\$
%Taking $k_l = x_l W^k$ and $v_l = x_l W^v$, we further write $\omega^{K, q} = (G^K)^{-1} \alpha^{K, q}$, where
%\$
%G^K & = \text{Ker}_K + L\lambda\cdot I_L = [\phi(x_l W^k)^\top \phi(x_{l'} W^k)]_{l, l' \in [L]} + L\lambda\cdot I_L \in \RR^{L\times L}\\
%\alpha^{K, q} & = \cS_K \text{ker}(q, \cdot)  = (\phi(q)^\top \phi(x_1W^k), \dots, \phi(q)^\top \phi(x_L W^k))^\top \in \RR^{L\times 1}
%\$
%Let $Q = [q_1^\top, \dots, q_L^\top]^\top$, the final output by CME is
%\$
%Z^{\text{CME}} = [(\hat{\mathcal{U}}_{V\,|\, K = q_1})^\top, \dots, (\hat{\mathcal{U}}_{V\,|\, K = q_L})^\top ]^\top = [(\omega^{K, q_1})^{\top}, \dots, (\omega^{K, q_L})^{\top}]^\top \Pi(V)
%\$
%We normalize the weight $\omega^{K, q}$ obtained by CME by its $1$-norm, i.e., $\tilde{\omega}^{K, q} = \omega^{K, q}/\|\omega^{K, q}\|_1$ and output
%\$
%Z = [z_1^\top, \dots, z_L^\top]^\top= [(\tilde{\omega}^{K, q_1})^{\top}, \dots, (\tilde{\omega}^{K, q_L})^{\top}]^\top \Pi(V)
%\$
%In sequel, we consider $\pi(v_l) \equiv v_l = x_l W^q$. We also consider the radial basis function (RBF) kernel applied to self-attention, which is
%\#\label{eq:rbf}
%\phi(xW)^\top \phi(x'W') = \text{ker}(x W, x' W') = \exp\{- \gamma^2 \cdot \|x W - x'W'\|_2^2\}.
%\#
%\begin{proposition}
%For the self-attention RBF kernel in \eqref{eq:rbf}, we have
%\$
%\text{ker}(x W, x' W')\cdot \|xW - x'W'\|_2 \leq 1/2\gamma.
%\$
%\end{proposition}
%We introduce the following assumption on the support of the inputs and the weights.
%\begin{assumption}\label{assumption:bound}
%Suppose that the input $x_l$ is bounded by $C_x$, i.e., $\|x_l\| \leq C_x$. Also, suppose that the query weight $W^q$ and the key weight $W^k$ have operator norms bounded by $C_W$.
%\end{assumption}
%
%We have the following lemma on the entry-wise Lipschitz continuity of the self-attention CME. We define the entry-wise self-attention CME as $\hat{\mathcal{U}}_{V\,|\, K = q}$.
%\begin{lemma}[Lipschitz Continuous Conditional Mean Embedding Self-Attention]\label{lemma:lip-condmean}
%Suppose that Assumption \ref{assumption:bound} holds. For any fixed $i \in [L]$, let $q = x_i W^Q$. We have empirical conditional mean embedding self-attention $\hat{\mathcal{U}}_{V\,|\, K = q}$ being $\lambda^{-1}\|W^v\|_{\rm op} \cdot(\gamma (1 + 2\lambda)\lambda^{-1} C_xC_W+1)$-Lipschitz continuous in $x_l$ for any $l \in [L]$.
%\end{lemma}
%\begin{proof}
%We consider $q = q_m = x_m W^q$. Differentiating $z_m$ with respect to $[x_l]_i = x_l e_i$, we have
%\$
%\frac{\partial z_m}{\partial x_l} = \frac{\partial ((\tilde{\omega}^{K, q_m})^{\top} V)}{\partial x_l} & = V^\top \frac{\partial \tilde{\omega}^{K, q_m}}{\partial x_l} + (\tilde{\omega}^{K, q_m})^\top\frac{\partial V}{\partial x_l}\\
%& = (W^v)^\top X^\top \frac{\partial \tilde{\omega}^{K, q_m}}{\partial x_l} + [\tilde{\omega}^{K, q_m}]_{l}\cdot I
%\$
%For the first term, we have
%\$
%\frac{\partial \omega^{K, q_m} }{\partial [x_l]_i} & = \frac{\partial [ (G^K)^{-1}\alpha^{K, q_m}]}{\partial [x_l]_i}\\
%& = \frac{\partial [(G^K)^{-1}]}{\partial [x_l]_i}\alpha^{K, q_m} + (G^K)^{-1}\frac{\partial  \alpha^{K, q_m}}{\partial [x_l]_i}\\
%& = (G^K)^{-1}\frac{\partial G^K}{\partial [x_l]_i}(G^K)^{-1}\alpha^{K, q_m} +(G^K)^{-1} \frac{\partial \alpha^{K, q_m}}{\partial [x_l]_i}\\
%& = (G^K)^{-1}\biggl( \frac{\partial G^K}{\partial [x_l]_i}\omega^{K, q_m} + \frac{\partial  \alpha^{K, q_m}}{\partial [x_l]_i}\biggr),
%\$
%which gives
%\$
%\frac{\partial \tilde{\omega}^{K, q_m} }{\partial [x_l]_i} & = \frac{1}{\|{\omega}^{K, q_m}\|_1} \cdot \frac{\partial \omega^{K, q_m}}{\partial [x_l]_i} + \frac{1}{\|{\omega}^{K, q_m}\|_1} \cdot\frac{\partial \|{\omega}^{K, q_m}\|_1}{\partial [x_l]_i}\cdot \tilde{\omega}^{K, q_m}\\
%& = \frac{1}{\|{\omega}^{K, q_m}\|_1} \cdot \frac{\partial \omega^{K, q_m}}{\partial [x_l]_i} + \frac{1}{\|{\omega}^{K, q_m}\|_1}\cdot \text{sgn}({\omega}^{K, q_m})^\top\frac{\partial {\omega}^{K, q_m}}{\partial [x_l]_i}\cdot \tilde{\omega}^{K, q_m}\\
%& =  (G^K)^{-1}\biggl( \frac{\partial G^K}{\partial [x_l]_i}\tilde{\omega}^{K, q_m} + \frac{1}{\|{\omega}^{K, q_m}\|_1} \cdot\frac{\partial  \alpha^{K, q_m}}{\partial [x_l]_i}\biggr) + \frac{1}{\|{\omega}^{K, q_m}\|_1}\cdot \text{sgn}({\omega}^{K, q_m})^\top\frac{\partial {\omega}^{K, q_m}}{\partial [x_l]_i}\cdot \tilde{\omega}^{K, q_m}
%\$
%Thus, we have
%\$
%\frac{\partial \hat{\mathcal{U}}_{V\,|\, K = q}}{\partial [x_l]_i} = \biggl((\omega^{K, q})^\top\frac{\partial G^K}{\partial [x_l]_i} + \frac{\partial  (\alpha^{K, q})^\top}{\partial [x_l]_i}\biggr)(G^K)^{-1}V + (\omega^{K, q})^\top\frac{\partial V}{\partial [x_l]_i} \in \RR^{1\times d}.
%\$
%For $q = x_mW^q$ for some $m \in [L]$, the Jacobian $\hat{J}_{m, l} = \partial z_m/ \partial x_l$ is
%\$
%\hat{J}_{m, l} = \biggl[\biggl(\frac{\partial \hat{\mathcal{U}}_{V\,|\, K = q}}{\partial [x_l]_1}\biggr)^\top, \dots, \biggl(\frac{\partial \hat{\mathcal{U}}_{V\,|\, K = q}}{\partial [x_l]_d}\biggr)^\top\biggr].
%\$
%To calculate the operator nomr of $J_{m, l}(X)$, we take $p_l = ([p_l]_1, \dots, [p_l]_d)^\top \in \RR^{d\times 1}$ and consider
%\$
% \hat{J}_{m, l}(X) p_l = \sum_{i = 1}^d [p_l]_i \cdot \frac{\partial \hat{\mathcal{U}}_{V\,|\, K = q_m}}{\partial [x_l]_i} \in \RR^{1\times d}.
%\$
%Thus, with $P = [p_1^\top , \dots, p_L^\top]^\top $, we have
%\$
%[\hat{J}_{m, 1}, \dots, \hat{J}_{m, L}] P = \sum_{l = 1}^L \hat{J}_{m, l}(X) p_l.
%\$
%\noindent{\bf Terms related to $\partial G^K/ \partial x_l$: } Let $A = [a_1^\top , \dots, a_L^\top]^\top  = (G^K)^{-1}XW^v \in \RR^{L\times d}$. We have
%\$
%A^\top \biggl(\sum_{l = 1}^L \sum_{i = 1}^d[p_l]_i\cdot \frac{\partial G^K}{\partial [x_l]_i}\biggr)\tilde{\omega}^{K, q_m} & = \sum_{l = 1}^L \sum_{l' = 1}^L  [\tilde{\omega}^{K, q_m}]_l \cdot [\text{Ker}]_{l, l'} (x_l - x_{l'})W^k(W^k)^\top p_l\cdot a_{l'}\\
%&\quad \qquad + \sum_{l = 1}^L \sum_{l' = 1}^L  [\tilde{\omega}^{K, q_m}]_{l'} \cdot  [\text{Ker}]_{l, l'} (x_{l'} - x_{l})W^k(W^k)^\top p_l\cdot a_{l}\\
%& = \sum_{l = 1}^L [\tilde{\omega}^{K, q_m}]_l \cdot \biggl[\sum_{l' = 1}^L   [\text{Ker}]_{l, l'} (x_l - x_{l'})W^k(W^k)^\top (p_l + p_{l'})\cdot a_{l'}\biggr].
%\$
%
%
%
%
%
%\begin{lemma}
%For self-attention RBF kernel defined in \eqref{eq:rbf}, we have
%\$
%\biggl\|\frac{\partial G^K}{\partial x_l}\biggr\| \leq \gamma\|W^k\|L, \quad \biggl\|\frac{\partial  (\alpha^{K, q})^\top}{\partial x_l}\biggr\| \leq 2\sqrt{L}\cdot \gamma \max\{\|W^q\|, \|W^k\|\}.
%\$
%\end{lemma}
%\begin{proof}
%See Appendix \ref{appendix:lip-condmean} for a detailed proof.
%\end{proof}
%
%Therefore, we have
%\$
%\biggl\|\frac{\partial \hat{\mathcal{U}}_{V\,|\, K = q}}{\partial x_l}\biggr\| & \leq  \biggl(\|(\omega^{K, q})^\top\| \cdot\biggl\|\frac{\partial G^K}{\partial x_l}\biggr\| + \biggl\|\frac{\partial  (\alpha^{K, q})^\top}{\partial x_l}\biggr\|\biggr)\|(G^K)^{-1}\|\|\Pi(V)\| + \|(\omega^{K, q})^\top\| \cdot\biggl\|\frac{\partial \Pi(V)}{\partial x_l}\biggr\|\\
%& \leq  \frac{\gamma (1 + 2\lambda)}{\lambda^2 \sqrt{L}}\max\{\|W^q\|, \|W^k\|\} \|W^v\| \sqrt{L} C_x + \|W^v\|/\lambda\sqrt{L}\\
%& \leq  \|W^v\|/\lambda \cdot\biggl( \frac{\gamma (1 + 2\lambda)}{\lambda} C_xC_W+1 \biggr).
%\$
%\end{proof}










==> optimization.tex <==
%!TEX root = iclr2023_conference.tex

\section{Optimization}\label{sec:opt}
In \S\ref{sec:opt-ap}, we study the optimization of transformer. Specifically, we show that when the transformer has sufficient expressive power, any stationary points for the optimization problem becomes globally optimal.




